Theory of Nuclear Magnetic Relaxation in Haldane Gap Materials: An Illustration of the Use of (1+1)-Dimensional Field Theory Techniques

A comprehensive theory of nuclear magnetic relaxation is developed for Haldane Gap materials using nonlinear sigma, boson and fermion models. We include a thorough discussion of of the effects of interchain couplings, nearest neighbour hyperfine couplings and crystal structure. We also introduce a new theory of impurities corresponding to broken chain ends weakly coupled to bulk magnons. The work is compared to recent experiments on NENP.

==> fig10 <==
%Figure10
%!PostScript
%%Creator: Xvgr version 2.10 - PJ Turner OGI-ESE
%%EndComments
/m {moveto} bind def
/l {lineto} bind def
/RJ {
 stringwidth neg exch neg exch
 rmoveto
} bind def
/CS {
 stringwidth
 2 div neg exch 2 div neg exch
 rmoveto
} bind def
0.25 0.25 scale
1 setlinecap
2450 0 translate
90 rotate
0.000000 0.000000 0.000000 setrgbcolor
1 setlinewidth
/Times-Italic findfont 
60 scalefont
 setfont
[] 0 setdash
528 420 m
528 2029 l
2642 2029 l
2642 420 l
528 420 l
stroke
[] 0 setdash
528 420 m
528 430 l
762 420 m
762 430 l
997 420 m
997 430 l
1232 420 m
1232 430 l
1467 420 m
1467 430 l
1702 420 m
1702 430 l
1937 420 m
1937 430 l
2172 420 m
2172 430 l
2407 420 m
2407 430 l
2642 420 m
2642 430 l
528 2029 m
528 2019 l
762 2029 m
762 2019 l
997 2029 m
997 2019 l
1232 2029 m
1232 2019 l
1467 2029 m
1467 2019 l
1702 2029 m
1702 2019 l
1937 2029 m
1937 2019 l
2172 2029 m
2172 2019 l
2407 2029 m
2407 2019 l
2642 2029 m
2642 2019 l
stroke
528 420 m
528 440 l
997 420 m
997 440 l
1467 420 m
1467 440 l
1937 420 m
1937 440 l
2407 420 m
2407 440 l
528 2029 m
528 2009 l
997 2029 m
997 2009 l
1467 2029 m
1467 2009 l
1937 2029 m
1937 2009 l
2407 2029 m
2407 2009 l
/Times-Italic findfont 
60 scalefont
 setfont
/Helvetica findfont 
60 scalefont
 setfont
stroke
528 370 m
gsave
528 370 translate
0 rotate
0 -20  m
(0.0) CS
(0.0) show
grestore
newpath
997 370 m
gsave
997 370 translate
0 rotate
0 -20  m
(20.0) CS
(20.0) show
grestore
newpath
1467 370 m
gsave
1467 370 translate
0 rotate
0 -20  m
(40.0) CS
(40.0) show
grestore
newpath
1937 370 m
gsave
1937 370 translate
0 rotate
0 -20  m
(60.0) CS
(60.0) show
grestore
newpath
2407 370 m
gsave
2407 370 translate
0 rotate
0 -20  m
(80.0) CS
(80.0) show
grestore
newpath
/Helvetica findfont 
60 scalefont
 setfont
1585 270 m
gsave
1585 270 translate
0 rotate
0 0  m
( q  \(Degrees\)) CS
/Symbol findfont 
60 scalefont
 setfont
( q ) show
/Helvetica findfont 
60 scalefont
 setfont
( \(Degrees\)) show
grestore
newpath
528 420 m
538 420 l
528 581 m
538 581 l
528 742 m
538 742 l
528 903 m
538 903 l
528 1064 m
538 1064 l
528 1224 m
538 1224 l
528 1386 m
538 1386 l
528 1546 m
538 1546 l
528 1708 m
538 1708 l
528 1868 m
538 1868 l
528 2029 m
538 2029 l
2642 420 m
2632 420 l
2642 581 m
2632 581 l
2642 742 m
2632 742 l
2642 903 m
2632 903 l
2642 1064 m
2632 1064 l
2642 1224 m
2632 1224 l
2642 1386 m
2632 1386 l
2642 1546 m
2632 1546 l
2642 1708 m
2632 1708 l
2642 1868 m
2632 1868 l
2642 2029 m
2632 2029 l
stroke
528 420 m
548 420 l
528 742 m
548 742 l
528 1064 m
548 1064 l
528 1386 m
548 1386 l
528 1708 m
548 1708 l
528 2029 m
548 2029 l
2642 420 m
2622 420 l
2642 742 m
2622 742 l
2642 1064 m
2622 1064 l
2642 1386 m
2622 1386 l
2642 1708 m
2622 1708 l
2642 2029 m
2622 2029 l
/Helvetica findfont 
60 scalefont
 setfont
stroke
490 420 m
gsave
490 420 translate
0 rotate
0 -20  m
(1.0) RJ
(1.0) show
grestore
newpath
490 742 m
gsave
490 742 translate
0 rotate
0 -20  m
(2.0) RJ
(2.0) show
grestore
newpath
490 1064 m
gsave
490 1064 translate
0 rotate
0 -20  m
(3.0) RJ
(3.0) show
grestore
newpath
490 1386 m
gsave
490 1386 translate
0 rotate
0 -20  m
(4.0) RJ
(4.0) show
grestore
newpath
490 1708 m
gsave
490 1708 translate
0 rotate
0 -20  m
(5.0) RJ
(5.0) show
grestore
newpath
490 2029 m
gsave
490 2029 translate
0 rotate
0 -20  m
(6.0) RJ
(6.0) show
grestore
newpath
/Helvetica findfont 
60 scalefont
 setfont
362 1224 m
gsave
362 1224 translate
90 rotate
0 0  m
(Resonance Field \(Tesla\)) CS
(Resonance Field \(Tesla\)) show
grestore
newpath
/Helvetica findfont 
90 scalefont
 setfont
1585 2197 m
gsave
1585 2197 translate
0 rotate
0 0  m
(ESR Resonance in NENP) CS
(ESR Resonance in NENP) show
grestore
newpath
649 587 12 0 360 arc
stroke
718 519 12 0 360 arc
stroke
788 581 12 0 360 arc
stroke
906 550 12 0 360 arc
stroke
1001 646 12 0 360 arc
stroke
1093 714 12 0 360 arc
stroke
1236 837 12 0 360 arc
stroke
1540 872 12 0 360 arc
stroke
1588 937 12 0 360 arc
stroke
1562 971 12 0 360 arc
stroke
1610 971 12 0 360 arc
stroke
1610 1070 12 0 360 arc
stroke
1702 1163 12 0 360 arc
stroke
1963 1320 12 0 360 arc
stroke
1963 1358 12 0 360 arc
stroke
1963 1420 12 0 360 arc
stroke
2293 1615 12 0 360 arc
stroke
2642 1711 12 0 360 arc
stroke
528 617 m
633 569 l
739 535 l
845 511 l
950 494 l
1056 484 l
1162 478 l
1267 477 l
1373 481 l
1479 490 l
1585 504 l
1690 526 l
1796 556 l
1902 599 l
2007 661 l
2113 749 l
2219 871 l
2324 1026 l
2430 1194 l
2536 1353 l
2642 1489 l
stroke
[40 20] 0 setdash
528 617 m
633 687 l
739 786 l
845 920 l
950 1082 l
1056 1249 l
1162 1401 l
1267 1528 l
1373 1624 l
1479 1694 l
1585 1742 l
1690 1772 l
1796 1790 l
1902 1797 l
2007 1796 l
2113 1785 l
2219 1764 l
2324 1728 l
2430 1674 l
2536 1595 l
2642 1489 l
stroke
[] 0 setdash
/Helvetica findfont 
60 scalefont
 setfont
/Helvetica findfont 
60 scalefont
 setfont
2466 1921 m
stroke
[] 0 setdash
2606 1921 12 0 360 arc
stroke
2641 1921 m
gsave
2641 1921 translate
0 rotate
0 -20  m
(Experiment) show
grestore
newpath
/Helvetica findfont 
60 scalefont
 setfont
2466 1847 m
2606 1847 l
stroke
2641 1847 m
gsave
2641 1847 translate
0 rotate
0 -20  m
(Chain 1) show
grestore
newpath
/Helvetica findfont 
60 scalefont
 setfont
[40 20] 0 setdash
2466 1773 m
2606 1773 l
stroke
[] 0 setdash
2641 1773 m
gsave
2641 1773 translate
0 rotate
0 -20  m
(Chain 2) show
grestore
newpath
showpage
%%Trailer


==> fig3 <==
%Figure3
%!PostScript
%%BoundingBox: 18 18 552 711
%%Creator: Xvgr version 2.10 - PJ Turner OGI-ESE
%%EndComments
/m {moveto} bind def
/l {lineto} bind def
/RJ {
 stringwidth neg exch neg exch
 rmoveto
} bind def
/CS {
 stringwidth
 2 div neg exch 2 div neg exch
 rmoveto
} bind def
0.25 0.25 scale
1 setlinecap
2450 0 translate
90 rotate
/Times-Italic findfont 
60 scalefont
 setfont
[] 0 setdash
519 420 m
519 2030 l
2595 2030 l
2595 420 l
519 420 l
stroke
[] 0 setdash
519 420 m
519 430 l
727 420 m
727 430 l
934 420 m
934 430 l
1142 420 m
1142 430 l
1349 420 m
1349 430 l
1557 420 m
1557 430 l
1765 420 m
1765 430 l
1972 420 m
1972 430 l
2180 420 m
2180 430 l
2387 420 m
2387 430 l
2595 420 m
2595 430 l
519 2030 m
519 2020 l
727 2030 m
727 2020 l
934 2030 m
934 2020 l
1142 2030 m
1142 2020 l
1349 2030 m
1349 2020 l
1557 2030 m
1557 2020 l
1765 2030 m
1765 2020 l
1972 2030 m
1972 2020 l
2180 2030 m
2180 2020 l
2387 2030 m
2387 2020 l
2595 2030 m
2595 2020 l
stroke
519 420 m
519 440 l
934 420 m
934 440 l
1349 420 m
1349 440 l
1765 420 m
1765 440 l
2180 420 m
2180 440 l
2595 420 m
2595 440 l
519 2030 m
519 2010 l
934 2030 m
934 2010 l
1349 2030 m
1349 2010 l
1765 2030 m
1765 2010 l
2180 2030 m
2180 2010 l
2595 2030 m
2595 2010 l
/Times-Italic findfont 
60 scalefont
 setfont
/Helvetica findfont 
60 scalefont
 setfont
stroke
519 370 m
gsave
519 370 translate
0 rotate
0 -20  m
(0.0) CS
(0.0) show
grestore
newpath
934 370 m
gsave
934 370 translate
0 rotate
0 -20  m
(2.0) CS
(2.0) show
grestore
newpath
1349 370 m
gsave
1349 370 translate
0 rotate
0 -20  m
(4.0) CS
(4.0) show
grestore
newpath
1765 370 m
gsave
1765 370 translate
0 rotate
0 -20  m
(6.0) CS
(6.0) show
grestore
newpath
2180 370 m
gsave
2180 370 translate
0 rotate
0 -20  m
(8.0) CS
(8.0) show
grestore
newpath
2595 370 m
gsave
2595 370 translate
0 rotate
0 -20  m
(10.0) CS
(10.0) show
grestore
newpath
/Helvetica findfont 
60 scalefont
 setfont
1557 270 m
gsave
1557 270 translate
0 rotate
0 0  m
(H \(Tesla\)) CS
(H \(Tesla\)) show
grestore
newpath
519 420 m
529 420 l
519 581 m
529 581 l
519 742 m
529 742 l
519 903 m
529 903 l
519 1064 m
529 1064 l
519 1225 m
529 1225 l
519 1386 m
529 1386 l
519 1546 m
529 1546 l
519 1708 m
529 1708 l
519 1868 m
529 1868 l
519 2030 m
529 2030 l
2595 420 m
2585 420 l
2595 581 m
2585 581 l
2595 742 m
2585 742 l
2595 903 m
2585 903 l
2595 1064 m
2585 1064 l
2595 1225 m
2585 1225 l
2595 1386 m
2585 1386 l
2595 1546 m
2585 1546 l
2595 1708 m
2585 1708 l
2595 1868 m
2585 1868 l
2595 2030 m
2585 2030 l
stroke
519 420 m
539 420 l
519 742 m
539 742 l
519 1064 m
539 1064 l
519 1386 m
539 1386 l
519 1708 m
539 1708 l
519 2030 m
539 2030 l
2595 420 m
2575 420 l
2595 742 m
2575 742 l
2595 1064 m
2575 1064 l
2595 1386 m
2575 1386 l
2595 1708 m
2575 1708 l
2595 2030 m
2575 2030 l
/Helvetica findfont 
60 scalefont
 setfont
stroke
481 420 m
gsave
481 420 translate
0 rotate
0 -20  m
(0.0) RJ
(0.0) show
grestore
newpath
481 742 m
gsave
481 742 translate
0 rotate
0 -20  m
(10.0) RJ
(10.0) show
grestore
newpath
481 1064 m
gsave
481 1064 translate
0 rotate
0 -20  m
(20.0) RJ
(20.0) show
grestore
newpath
481 1386 m
gsave
481 1386 translate
0 rotate
0 -20  m
(30.0) RJ
(30.0) show
grestore
newpath
481 1708 m
gsave
481 1708 translate
0 rotate
0 -20  m
(40.0) RJ
(40.0) show
grestore
newpath
481 2030 m
gsave
481 2030 translate
0 rotate
0 -20  m
(50.0) RJ
(50.0) show
grestore
newpath
/Helvetica findfont 
60 scalefont
 setfont
308 1225 m
gsave
308 1225 translate
90 rotate
0 0  m
(F\(h,T\) \(s-1\)) CS
(F\(h,T\) \(s) show
/Helvetica findfont 
36 scalefont
 setfont
0 36 rmoveto
(-1) show
/Helvetica findfont 
60 scalefont
 setfont
0 -36 rmoveto
(\)) show
grestore
newpath
/Helvetica findfont 
90 scalefont
 setfont
1557 2198 m
gsave
1557 2198 translate
0 rotate
0 0  m
(Boson F\(h,T\):) CS
(Boson F\(h,T\):) show
grestore
newpath
/Helvetica findfont 
60 scalefont
 setfont
1557 2080 m
gsave
1557 2080 translate
0 rotate
0 0  m
(Contributions From The Uniform Part of the Spin   ) CS
(Contributions From The Uniform Part of the Spin   ) show
grestore
newpath
540 480 m
561 482 l
582 485 l
602 489 l
623 494 l
644 500 l
665 507 l
685 516 l
706 525 l
727 534 l
748 545 l
768 557 l
789 569 l
810 582 l
831 596 l
851 611 l
872 627 l
893 644 l
914 662 l
934 680 l
955 700 l
976 721 l
997 744 l
1017 768 l
1038 794 l
1059 822 l
1080 854 l
1100 889 l
1121 930 l
1142 977 l
1163 1035 l
1183 1111 l
1204 1222 l
1225 1466 l
1246 1394 l
1266 1223 l
1287 1140 l
1308 1088 l
1329 1050 l
1349 1022 l
1370 1001 l
1391 984 l
1412 972 l
1432 962 l
1453 954 l
1474 948 l
1495 944 l
1515 941 l
1536 940 l
1557 939 l
1578 939 l
1599 940 l
1619 941 l
1640 943 l
1661 946 l
1682 948 l
1702 952 l
1723 955 l
1744 959 l
1765 963 l
1785 967 l
1806 972 l
1827 976 l
1848 981 l
1868 986 l
1889 991 l
1910 997 l
1931 1002 l
1951 1008 l
1972 1013 l
1993 1019 l
2014 1025 l
2034 1031 l
2055 1038 l
2076 1044 l
2097 1051 l
2117 1058 l
2138 1066 l
2159 1073 l
2180 1081 l
2200 1089 l
2221 1098 l
2242 1107 l
2263 1116 l
2283 1126 l
2304 1137 l
2325 1148 l
2346 1160 l
2366 1173 l
2387 1187 l
stroke
[4 8] 0 setdash
540 525 m
561 527 l
582 531 l
602 535 l
623 541 l
644 548 l
665 555 l
685 564 l
706 574 l
727 585 l
748 597 l
768 609 l
789 623 l
810 638 l
831 653 l
851 669 l
872 687 l
893 705 l
914 724 l
934 745 l
955 766 l
976 789 l
997 814 l
1017 840 l
1038 868 l
1059 898 l
1080 931 l
1100 968 l
1121 1010 l
1142 1058 l
1163 1117 l
1183 1193 l
1204 1304 l
1225 1545 l
1246 1475 l
1266 1307 l
1287 1226 l
1308 1174 l
1329 1137 l
1349 1109 l
1370 1087 l
1391 1069 l
1412 1055 l
1432 1044 l
1453 1035 l
1474 1027 l
1495 1022 l
1515 1017 l
1536 1013 l
1557 1011 l
1578 1009 l
1599 1008 l
1619 1007 l
1640 1007 l
1661 1008 l
1682 1009 l
1702 1010 l
1723 1012 l
1744 1014 l
1765 1016 l
1785 1018 l
1806 1021 l
1827 1024 l
1848 1027 l
1868 1030 l
1889 1034 l
1910 1037 l
1931 1041 l
1951 1045 l
1972 1049 l
1993 1053 l
2014 1058 l
2034 1062 l
2055 1067 l
2076 1071 l
2097 1076 l
2117 1081 l
2138 1086 l
2159 1091 l
2180 1096 l
2200 1102 l
2221 1107 l
2242 1113 l
2263 1119 l
2283 1125 l
2304 1132 l
2325 1138 l
2346 1145 l
2366 1153 l
2387 1160 l
stroke
[] 0 setdash
[20 20] 0 setdash
540 652 m
561 654 l
582 657 l
602 662 l
623 668 l
644 676 l
665 684 l
685 694 l
706 704 l
727 716 l
748 729 l
768 743 l
789 758 l
810 774 l
831 790 l
851 808 l
872 827 l
893 846 l
914 867 l
934 889 l
955 912 l
976 936 l
997 961 l
1017 988 l
1038 1017 l
1059 1048 l
1080 1082 l
1100 1119 l
1121 1160 l
1142 1208 l
1163 1266 l
1183 1339 l
1204 1447 l
1225 1682 l
1246 1614 l
1266 1451 l
1287 1373 l
1308 1323 l
1329 1287 l
1349 1259 l
1370 1237 l
1391 1219 l
1412 1204 l
1432 1191 l
1453 1180 l
1474 1170 l
1495 1162 l
1515 1154 l
1536 1147 l
1557 1141 l
1578 1136 l
1599 1131 l
1619 1126 l
1640 1122 l
1661 1118 l
1682 1114 l
1702 1110 l
1723 1107 l
1744 1104 l
1765 1101 l
1785 1098 l
1806 1095 l
1827 1092 l
1848 1090 l
1868 1087 l
1889 1085 l
1910 1082 l
1931 1079 l
1951 1077 l
1972 1074 l
1993 1072 l
2014 1069 l
2034 1067 l
2055 1064 l
2076 1062 l
2097 1059 l
2117 1057 l
2138 1054 l
2159 1052 l
2180 1050 l
2200 1047 l
2221 1045 l
2242 1043 l
2263 1040 l
2283 1038 l
2304 1036 l
2325 1035 l
2346 1033 l
2366 1032 l
2387 1031 l
stroke
[] 0 setdash
7 setlinewidth
540 501 m
561 554 l
582 622 l
602 693 l
623 758 l
644 812 l
665 855 l
685 889 l
706 915 l
727 934 l
748 949 l
768 961 l
789 969 l
810 976 l
831 981 l
851 985 l
872 988 l
893 990 l
914 992 l
934 993 l
955 994 l
976 995 l
997 995 l
1017 995 l
1038 995 l
1059 995 l
1080 994 l
1100 994 l
1121 993 l
1142 993 l
1163 992 l
1183 991 l
1204 990 l
1225 990 l
1246 989 l
1266 988 l
1287 987 l
1308 986 l
1329 985 l
1349 985 l
1370 984 l
1391 983 l
1412 982 l
1432 982 l
1453 981 l
1474 980 l
1495 980 l
1515 979 l
1536 979 l
1557 979 l
1578 979 l
1599 979 l
1619 979 l
1640 979 l
1661 980 l
1682 980 l
1702 981 l
1723 982 l
1744 983 l
1765 985 l
1785 987 l
1806 989 l
1827 992 l
1848 995 l
1868 999 l
1889 1004 l
1910 1009 l
1931 1015 l
1951 1022 l
1972 1030 l
1993 1040 l
2014 1051 l
2034 1064 l
2055 1080 l
2076 1098 l
2097 1120 l
2117 1146 l
2138 1177 l
2159 1215 l
2180 1262 l
2200 1322 l
2221 1399 l
2242 1500 l
2263 1640 l
2283 1842 l
2296 2030 l
stroke
1 setlinewidth
7 setlinewidth
[4 8] 0 setdash
540 548 m
561 607 l
582 682 l
602 760 l
623 829 l
644 887 l
665 933 l
685 967 l
706 993 l
727 1011 l
748 1023 l
768 1032 l
789 1038 l
810 1042 l
831 1044 l
851 1045 l
872 1045 l
893 1045 l
914 1044 l
934 1043 l
955 1042 l
976 1041 l
997 1040 l
1017 1039 l
1038 1038 l
1059 1037 l
1080 1036 l
1100 1035 l
1121 1034 l
1142 1033 l
1163 1033 l
1183 1032 l
1204 1031 l
1225 1031 l
1246 1030 l
1266 1030 l
1287 1030 l
1308 1030 l
1329 1030 l
1349 1030 l
1370 1030 l
1391 1030 l
1412 1030 l
1432 1031 l
1453 1032 l
1474 1033 l
1495 1034 l
1515 1035 l
1536 1037 l
1557 1038 l
1578 1040 l
1599 1043 l
1619 1045 l
1640 1048 l
1661 1052 l
1682 1055 l
1702 1060 l
1723 1064 l
1744 1070 l
1765 1076 l
1785 1082 l
1806 1090 l
1827 1098 l
1848 1107 l
1868 1117 l
1889 1129 l
1910 1142 l
1931 1157 l
1951 1173 l
1972 1192 l
1993 1213 l
2014 1237 l
2034 1265 l
2055 1297 l
2076 1335 l
2097 1378 l
2117 1430 l
2138 1492 l
2159 1566 l
2180 1658 l
2200 1772 l
2221 1919 l
2233 2030 l
stroke
[] 0 setdash
1 setlinewidth
7 setlinewidth
[20 20] 0 setdash
540 693 m
561 767 l
582 864 l
602 964 l
623 1056 l
644 1133 l
665 1194 l
685 1240 l
706 1274 l
727 1299 l
748 1315 l
768 1326 l
789 1332 l
810 1335 l
831 1336 l
851 1334 l
872 1332 l
893 1329 l
914 1326 l
934 1322 l
955 1318 l
976 1315 l
997 1311 l
1017 1308 l
1038 1305 l
1059 1303 l
1080 1301 l
1100 1300 l
1121 1299 l
1142 1299 l
1163 1299 l
1183 1299 l
1204 1300 l
1225 1302 l
1246 1304 l
1266 1307 l
1287 1311 l
1308 1315 l
1329 1320 l
1349 1325 l
1370 1331 l
1391 1337 l
1412 1345 l
1432 1353 l
1453 1362 l
1474 1371 l
1495 1382 l
1515 1393 l
1536 1406 l
1557 1419 l
1578 1434 l
1599 1449 l
1619 1466 l
1640 1485 l
1661 1505 l
1682 1526 l
1702 1550 l
1723 1575 l
1744 1603 l
1765 1632 l
1785 1665 l
1806 1700 l
1827 1739 l
1848 1782 l
1868 1828 l
1889 1880 l
1910 1937 l
1931 2000 l
1939 2030 l
stroke
[] 0 setdash
1 setlinewidth
/Helvetica findfont 
60 scalefont
 setfont
/Helvetica findfont 
60 scalefont
 setfont
2438 1813 m
2578 1813 l
stroke
2613 1813 m
gsave
2613 1813 translate
0 rotate
0 -20  m
(H) show
/Helvetica findfont 
36 scalefont
 setfont
0 -18 rmoveto
(||a) show
/Helvetica findfont 
60 scalefont
 setfont
0 18 rmoveto
( at 1.4 K) show
grestore
newpath
/Helvetica findfont 
60 scalefont
 setfont
[4 8] 0 setdash
2438 1739 m
2578 1739 l
stroke
[] 0 setdash
2613 1739 m
gsave
2613 1739 translate
0 rotate
0 -20  m
(H) show
/Helvetica findfont 
36 scalefont
 setfont
0 -18 rmoveto
(||a) show
/Helvetica findfont 
60 scalefont
 setfont
0 18 rmoveto
( at 2.0 K) show
grestore
newpath
/Helvetica findfont 
60 scalefont
 setfont
[20 20] 0 setdash
2438 1665 m
2578 1665 l
stroke
[] 0 setdash
2613 1665 m
gsave
2613 1665 translate
0 rotate
0 -20  m
(H) show
/Helvetica findfont 
36 scalefont
 setfont
0 -18 rmoveto
(||a) show
/Helvetica findfont 
60 scalefont
 setfont
0 18 rmoveto
( at 4.2 K) show
grestore
newpath
/Helvetica findfont 
60 scalefont
 setfont
7 setlinewidth
2438 1591 m
2578 1591 l
stroke
1 setlinewidth
2613 1591 m
gsave
2613 1591 translate
0 rotate
0 -20  m
(H) show
/Helvetica findfont 
36 scalefont
 setfont
0 -18 rmoveto
(||b) show
/Helvetica findfont 
60 scalefont
 setfont
0 18 rmoveto
( at 1.4 K) show
grestore
newpath
/Helvetica findfont 
60 scalefont
 setfont
[4 8] 0 setdash
7 setlinewidth
2438 1517 m
2578 1517 l
stroke
[] 0 setdash
1 setlinewidth
2613 1517 m
gsave
2613 1517 translate
0 rotate
0 -20  m
(H) show
/Helvetica findfont 
36 scalefont
 setfont
0 -18 rmoveto
(||b) show
/Helvetica findfont 
60 scalefont
 setfont
0 18 rmoveto
( at 2.0 K) show
grestore
newpath
/Helvetica findfont 
60 scalefont
 setfont
[20 20] 0 setdash
7 setlinewidth
2438 1443 m
2578 1443 l
stroke
[] 0 setdash
1 setlinewidth
2613 1443 m
gsave
2613 1443 translate
0 rotate
0 -20  m
(H) show
/Helvetica findfont 
36 scalefont
 setfont
0 -18 rmoveto
(||b) show
/Helvetica findfont 
60 scalefont
 setfont
0 18 rmoveto
( at 4.2 K) show
grestore
newpath
showpage
%%Trailer


==> fig4 <==
%Figure4
%!PostScript
%%BoundingBox: 18 18 552 711
%%Creator: Xvgr version 2.10 - PJ Turner OGI-ESE
%%EndComments
/m {moveto} bind def
/l {lineto} bind def
/RJ {
 stringwidth neg exch neg exch
 rmoveto
} bind def
/CS {
 stringwidth
 2 div neg exch 2 div neg exch
 rmoveto
} bind def
0.25 0.25 scale
1 setlinecap
2450 0 translate
90 rotate
/Times-Italic findfont 
60 scalefont
 setfont
[] 0 setdash
519 420 m
519 2030 l
2595 2030 l
2595 420 l
519 420 l
stroke
[] 0 setdash
519 420 m
519 430 l
727 420 m
727 430 l
934 420 m
934 430 l
1142 420 m
1142 430 l
1349 420 m
1349 430 l
1557 420 m
1557 430 l
1765 420 m
1765 430 l
1972 420 m
1972 430 l
2180 420 m
2180 430 l
2387 420 m
2387 430 l
2595 420 m
2595 430 l
519 2030 m
519 2020 l
727 2030 m
727 2020 l
934 2030 m
934 2020 l
1142 2030 m
1142 2020 l
1349 2030 m
1349 2020 l
1557 2030 m
1557 2020 l
1765 2030 m
1765 2020 l
1972 2030 m
1972 2020 l
2180 2030 m
2180 2020 l
2387 2030 m
2387 2020 l
2595 2030 m
2595 2020 l
stroke
519 420 m
519 440 l
934 420 m
934 440 l
1349 420 m
1349 440 l
1765 420 m
1765 440 l
2180 420 m
2180 440 l
2595 420 m
2595 440 l
519 2030 m
519 2010 l
934 2030 m
934 2010 l
1349 2030 m
1349 2010 l
1765 2030 m
1765 2010 l
2180 2030 m
2180 2010 l
2595 2030 m
2595 2010 l
/Times-Italic findfont 
60 scalefont
 setfont
/Helvetica findfont 
60 scalefont
 setfont
stroke
519 370 m
gsave
519 370 translate
0 rotate
0 -20  m
(0.0) CS
(0.0) show
grestore
newpath
934 370 m
gsave
934 370 translate
0 rotate
0 -20  m
(2.0) CS
(2.0) show
grestore
newpath
1349 370 m
gsave
1349 370 translate
0 rotate
0 -20  m
(4.0) CS
(4.0) show
grestore
newpath
1765 370 m
gsave
1765 370 translate
0 rotate
0 -20  m
(6.0) CS
(6.0) show
grestore
newpath
2180 370 m
gsave
2180 370 translate
0 rotate
0 -20  m
(8.0) CS
(8.0) show
grestore
newpath
2595 370 m
gsave
2595 370 translate
0 rotate
0 -20  m
(10.0) CS
(10.0) show
grestore
newpath
/Helvetica findfont 
60 scalefont
 setfont
1557 270 m
gsave
1557 270 translate
0 rotate
0 0  m
(H \(Tesla\)) CS
(H \(Tesla\)) show
grestore
newpath
519 420 m
529 420 l
519 581 m
529 581 l
519 742 m
529 742 l
519 903 m
529 903 l
519 1064 m
529 1064 l
519 1225 m
529 1225 l
519 1386 m
529 1386 l
519 1546 m
529 1546 l
519 1708 m
529 1708 l
519 1868 m
529 1868 l
519 2030 m
529 2030 l
2595 420 m
2585 420 l
2595 581 m
2585 581 l
2595 742 m
2585 742 l
2595 903 m
2585 903 l
2595 1064 m
2585 1064 l
2595 1225 m
2585 1225 l
2595 1386 m
2585 1386 l
2595 1546 m
2585 1546 l
2595 1708 m
2585 1708 l
2595 1868 m
2585 1868 l
2595 2030 m
2585 2030 l
stroke
519 420 m
539 420 l
519 742 m
539 742 l
519 1064 m
539 1064 l
519 1386 m
539 1386 l
519 1708 m
539 1708 l
519 2030 m
539 2030 l
2595 420 m
2575 420 l
2595 742 m
2575 742 l
2595 1064 m
2575 1064 l
2595 1386 m
2575 1386 l
2595 1708 m
2575 1708 l
2595 2030 m
2575 2030 l
/Helvetica findfont 
60 scalefont
 setfont
stroke
481 420 m
gsave
481 420 translate
0 rotate
0 -20  m
(0.0) RJ
(0.0) show
grestore
newpath
481 742 m
gsave
481 742 translate
0 rotate
0 -20  m
(10.0) RJ
(10.0) show
grestore
newpath
481 1064 m
gsave
481 1064 translate
0 rotate
0 -20  m
(20.0) RJ
(20.0) show
grestore
newpath
481 1386 m
gsave
481 1386 translate
0 rotate
0 -20  m
(30.0) RJ
(30.0) show
grestore
newpath
481 1708 m
gsave
481 1708 translate
0 rotate
0 -20  m
(40.0) RJ
(40.0) show
grestore
newpath
481 2030 m
gsave
481 2030 translate
0 rotate
0 -20  m
(50.0) RJ
(50.0) show
grestore
newpath
/Helvetica findfont 
60 scalefont
 setfont
308 1225 m
gsave
308 1225 translate
90 rotate
0 0  m
(F\(h,T\) \(s-1\)) CS
(F\(h,T\) \(s) show
/Helvetica findfont 
36 scalefont
 setfont
0 36 rmoveto
(-1) show
/Helvetica findfont 
60 scalefont
 setfont
0 -36 rmoveto
(\)) show
grestore
newpath
/Helvetica findfont 
90 scalefont
 setfont
1557 2198 m
gsave
1557 2198 translate
0 rotate
0 0  m
(Boson F\(h,T\):) CS
(Boson F\(h,T\):) show
grestore
newpath
/Helvetica findfont 
60 scalefont
 setfont
1557 2080 m
gsave
1557 2080 translate
0 rotate
0 0  m
(Contributions From The Uniform Part of the Spin   ) CS
(Contributions From The Uniform Part of the Spin   ) show
grestore
newpath
540 480 m
561 481 l
582 482 l
602 484 l
623 486 l
644 489 l
665 493 l
685 496 l
706 501 l
727 505 l
748 510 l
768 515 l
789 521 l
810 526 l
831 533 l
851 539 l
872 546 l
893 553 l
914 560 l
934 567 l
955 575 l
976 582 l
997 590 l
1017 598 l
1038 606 l
1059 614 l
1080 623 l
1100 631 l
1121 640 l
1142 648 l
1163 657 l
1183 666 l
1204 674 l
1225 683 l
1246 692 l
1266 700 l
1287 709 l
1308 718 l
1329 726 l
1349 735 l
1370 744 l
1391 752 l
1412 761 l
1432 769 l
1453 778 l
1474 786 l
1495 795 l
1515 803 l
1536 811 l
1557 820 l
1578 828 l
1599 836 l
1619 845 l
1640 853 l
1661 861 l
1682 869 l
1702 878 l
1723 886 l
1744 895 l
1765 903 l
1785 912 l
1806 921 l
1827 930 l
1848 939 l
1868 948 l
1889 958 l
1910 968 l
1931 978 l
1951 988 l
1972 999 l
1993 1010 l
2014 1022 l
2034 1034 l
2055 1047 l
2076 1061 l
2097 1075 l
2117 1091 l
2138 1108 l
2159 1126 l
2180 1145 l
2200 1167 l
2221 1191 l
2242 1217 l
2263 1247 l
2283 1282 l
2304 1323 l
2325 1375 l
2346 1447 l
2366 1577 l
2381 2030 l
stroke
[4 8] 0 setdash
540 525 m
561 526 l
582 527 l
602 529 l
623 532 l
644 534 l
665 537 l
685 541 l
706 545 l
727 549 l
748 554 l
768 559 l
789 564 l
810 569 l
831 575 l
851 581 l
872 587 l
893 594 l
914 601 l
934 607 l
955 614 l
976 622 l
997 629 l
1017 637 l
1038 644 l
1059 652 l
1080 660 l
1100 668 l
1121 676 l
1142 684 l
1163 692 l
1183 700 l
1204 708 l
1225 716 l
1246 724 l
1266 733 l
1287 741 l
1308 749 l
1329 757 l
1349 765 l
1370 773 l
1391 781 l
1412 789 l
1432 797 l
1453 805 l
1474 813 l
1495 821 l
1515 829 l
1536 837 l
1557 845 l
1578 853 l
1599 860 l
1619 868 l
1640 876 l
1661 883 l
1682 891 l
1702 899 l
1723 906 l
1744 914 l
1765 922 l
1785 930 l
1806 937 l
1827 945 l
1848 953 l
1868 961 l
1889 969 l
1910 977 l
1931 985 l
1951 993 l
1972 1002 l
1993 1010 l
2014 1019 l
2034 1028 l
2055 1038 l
2076 1047 l
2097 1057 l
2117 1068 l
2138 1079 l
2159 1090 l
2180 1102 l
2200 1116 l
2221 1130 l
2242 1146 l
2263 1165 l
2283 1187 l
2304 1214 l
2325 1252 l
2346 1312 l
2366 1436 l
2384 2030 l
stroke
[] 0 setdash
[20 20] 0 setdash
540 651 m
561 652 l
582 653 l
602 655 l
623 657 l
644 660 l
665 662 l
685 666 l
706 669 l
727 673 l
748 677 l
768 681 l
789 686 l
810 691 l
831 696 l
851 701 l
872 706 l
893 712 l
914 717 l
934 723 l
955 729 l
976 735 l
997 741 l
1017 747 l
1038 753 l
1059 759 l
1080 765 l
1100 771 l
1121 777 l
1142 783 l
1163 789 l
1183 795 l
1204 800 l
1225 806 l
1246 812 l
1266 817 l
1287 823 l
1308 828 l
1329 833 l
1349 839 l
1370 843 l
1391 848 l
1412 853 l
1432 858 l
1453 862 l
1474 867 l
1495 871 l
1515 875 l
1536 879 l
1557 882 l
1578 886 l
1599 890 l
1619 893 l
1640 896 l
1661 899 l
1682 902 l
1702 905 l
1723 908 l
1744 910 l
1765 913 l
1785 915 l
1806 917 l
1827 919 l
1848 921 l
1868 923 l
1889 925 l
1910 927 l
1931 928 l
1951 930 l
1972 932 l
1993 933 l
2014 935 l
2034 937 l
2055 939 l
2076 941 l
2097 943 l
2117 946 l
2138 949 l
2159 952 l
2180 957 l
2200 962 l
2221 970 l
2242 979 l
2263 991 l
2283 1008 l
2304 1032 l
2325 1069 l
2346 1133 l
2366 1274 l
2386 2030 l
stroke
[] 0 setdash
7 setlinewidth
540 501 m
561 554 l
582 622 l
602 693 l
623 758 l
644 812 l
665 855 l
685 889 l
706 915 l
727 934 l
748 949 l
768 961 l
789 969 l
810 976 l
831 981 l
851 985 l
872 988 l
893 990 l
914 992 l
934 993 l
955 994 l
976 995 l
997 995 l
1017 995 l
1038 995 l
1059 995 l
1080 994 l
1100 994 l
1121 993 l
1142 993 l
1163 992 l
1183 991 l
1204 990 l
1225 990 l
1246 989 l
1266 988 l
1287 987 l
1308 986 l
1329 985 l
1349 985 l
1370 984 l
1391 983 l
1412 982 l
1432 982 l
1453 981 l
1474 980 l
1495 980 l
1515 979 l
1536 979 l
1557 979 l
1578 979 l
1599 979 l
1619 979 l
1640 979 l
1661 980 l
1682 980 l
1702 981 l
1723 982 l
1744 983 l
1765 985 l
1785 987 l
1806 989 l
1827 992 l
1848 995 l
1868 999 l
1889 1004 l
1910 1009 l
1931 1015 l
1951 1022 l
1972 1030 l
1993 1040 l
2014 1051 l
2034 1064 l
2055 1080 l
2076 1098 l
2097 1120 l
2117 1146 l
2138 1177 l
2159 1215 l
2180 1262 l
2200 1322 l
2221 1399 l
2242 1500 l
2263 1640 l
2283 1842 l
2296 2030 l
stroke
1 setlinewidth
7 setlinewidth
[4 8] 0 setdash
540 548 m
561 607 l
582 682 l
602 760 l
623 829 l
644 887 l
665 933 l
685 967 l
706 993 l
727 1011 l
748 1023 l
768 1032 l
789 1038 l
810 1042 l
831 1044 l
851 1045 l
872 1045 l
893 1045 l
914 1044 l
934 1043 l
955 1042 l
976 1041 l
997 1040 l
1017 1039 l
1038 1038 l
1059 1037 l
1080 1036 l
1100 1035 l
1121 1034 l
1142 1033 l
1163 1033 l
1183 1032 l
1204 1031 l
1225 1031 l
1246 1030 l
1266 1030 l
1287 1030 l
1308 1030 l
1329 1030 l
1349 1030 l
1370 1030 l
1391 1030 l
1412 1030 l
1432 1031 l
1453 1032 l
1474 1033 l
1495 1034 l
1515 1035 l
1536 1037 l
1557 1038 l
1578 1040 l
1599 1043 l
1619 1045 l
1640 1048 l
1661 1052 l
1682 1055 l
1702 1060 l
1723 1064 l
1744 1070 l
1765 1076 l
1785 1082 l
1806 1090 l
1827 1098 l
1848 1107 l
1868 1117 l
1889 1129 l
1910 1142 l
1931 1157 l
1951 1173 l
1972 1192 l
1993 1213 l
2014 1237 l
2034 1265 l
2055 1297 l
2076 1335 l
2097 1378 l
2117 1430 l
2138 1492 l
2159 1566 l
2180 1658 l
2200 1772 l
2221 1919 l
2233 2030 l
stroke
[] 0 setdash
1 setlinewidth
7 setlinewidth
[20 20] 0 setdash
540 693 m
561 767 l
582 864 l
602 964 l
623 1056 l
644 1133 l
665 1194 l
685 1240 l
706 1274 l
727 1299 l
748 1315 l
768 1326 l
789 1332 l
810 1335 l
831 1336 l
851 1334 l
872 1332 l
893 1329 l
914 1326 l
934 1322 l
955 1318 l
976 1315 l
997 1311 l
1017 1308 l
1038 1305 l
1059 1303 l
1080 1301 l
1100 1300 l
1121 1299 l
1142 1299 l
1163 1299 l
1183 1299 l
1204 1300 l
1225 1302 l
1246 1304 l
1266 1307 l
1287 1311 l
1308 1315 l
1329 1320 l
1349 1325 l
1370 1331 l
1391 1337 l
1412 1345 l
1432 1353 l
1453 1362 l
1474 1371 l
1495 1382 l
1515 1393 l
1536 1406 l
1557 1419 l
1578 1434 l
1599 1449 l
1619 1466 l
1640 1485 l
1661 1505 l
1682 1526 l
1702 1550 l
1723 1575 l
1744 1603 l
1765 1632 l
1785 1665 l
1806 1700 l
1827 1739 l
1848 1782 l
1868 1828 l
1889 1880 l
1910 1937 l
1931 2000 l
1939 2030 l
stroke
[] 0 setdash
1 setlinewidth
/Helvetica findfont 
60 scalefont
 setfont
/Helvetica findfont 
60 scalefont
 setfont
2438 1813 m
2578 1813 l
stroke
2613 1813 m
gsave
2613 1813 translate
0 rotate
0 -20  m
(H) show
/Helvetica findfont 
36 scalefont
 setfont
0 -18 rmoveto
(||c) show
/Helvetica findfont 
60 scalefont
 setfont
0 18 rmoveto
( at 1.4 K) show
grestore
newpath
/Helvetica findfont 
60 scalefont
 setfont
[4 8] 0 setdash
2438 1739 m
2578 1739 l
stroke
[] 0 setdash
2613 1739 m
gsave
2613 1739 translate
0 rotate
0 -20  m
(H) show
/Helvetica findfont 
36 scalefont
 setfont
0 -18 rmoveto
(||c) show
/Helvetica findfont 
60 scalefont
 setfont
0 18 rmoveto
( at 2.0 K) show
grestore
newpath
/Helvetica findfont 
60 scalefont
 setfont
[20 20] 0 setdash
2438 1665 m
2578 1665 l
stroke
[] 0 setdash
2613 1665 m
gsave
2613 1665 translate
0 rotate
0 -20  m
(H) show
/Helvetica findfont 
36 scalefont
 setfont
0 -18 rmoveto
(||c) show
/Helvetica findfont 
60 scalefont
 setfont
0 18 rmoveto
( at 4.2 K) show
grestore
newpath
/Helvetica findfont 
60 scalefont
 setfont
7 setlinewidth
2438 1591 m
2578 1591 l
stroke
1 setlinewidth
2613 1591 m
gsave
2613 1591 translate
0 rotate
0 -20  m
(H) show
/Helvetica findfont 
36 scalefont
 setfont
0 -18 rmoveto
(||b) show
/Helvetica findfont 
60 scalefont
 setfont
0 18 rmoveto
( at 1.4 K) show
grestore
newpath
/Helvetica findfont 
60 scalefont
 setfont
[4 8] 0 setdash
7 setlinewidth
2438 1517 m
2578 1517 l
stroke
[] 0 setdash
1 setlinewidth
2613 1517 m
gsave
2613 1517 translate
0 rotate
0 -20  m
(H) show
/Helvetica findfont 
36 scalefont
 setfont
0 -18 rmoveto
(||b) show
/Helvetica findfont 
60 scalefont
 setfont
0 18 rmoveto
( at 2.0 K) show
grestore
newpath
/Helvetica findfont 
60 scalefont
 setfont
[20 20] 0 setdash
7 setlinewidth
2438 1443 m
2578 1443 l
stroke
[] 0 setdash
1 setlinewidth
2613 1443 m
gsave
2613 1443 translate
0 rotate
0 -20  m
(H) show
/Helvetica findfont 
36 scalefont
 setfont
0 -18 rmoveto
(||b) show
/Helvetica findfont 
60 scalefont
 setfont
0 18 rmoveto
( at 4.2 K) show
grestore
newpath
showpage
%%Trailer


==> fig5 <==
%Figure5
%!PostScript
%%Creator: Xvgr version 2.10 - PJ Turner OGI-ESE
%%EndComments
/m {moveto} bind def
/l {lineto} bind def
/RJ {
 stringwidth neg exch neg exch
 rmoveto
} bind def
/CS {
 stringwidth
 2 div neg exch 2 div neg exch
 rmoveto
} bind def
0.25 0.25 scale
1 setlinecap
2450 0 translate
90 rotate
/Times-Italic findfont 
60 scalefont
 setfont
[] 0 setdash
528 420 m
528 2030 l
2642 2030 l
2642 420 l
528 420 l
stroke
[] 0 setdash
528 420 m
528 430 l
739 420 m
739 430 l
950 420 m
950 430 l
1162 420 m
1162 430 l
1373 420 m
1373 430 l
1585 420 m
1585 430 l
1796 420 m
1796 430 l
2007 420 m
2007 430 l
2219 420 m
2219 430 l
2430 420 m
2430 430 l
2642 420 m
2642 430 l
528 2030 m
528 2020 l
739 2030 m
739 2020 l
950 2030 m
950 2020 l
1162 2030 m
1162 2020 l
1373 2030 m
1373 2020 l
1585 2030 m
1585 2020 l
1796 2030 m
1796 2020 l
2007 2030 m
2007 2020 l
2219 2030 m
2219 2020 l
2430 2030 m
2430 2020 l
2642 2030 m
2642 2020 l
stroke
528 420 m
528 440 l
950 420 m
950 440 l
1373 420 m
1373 440 l
1796 420 m
1796 440 l
2219 420 m
2219 440 l
2642 420 m
2642 440 l
528 2030 m
528 2010 l
950 2030 m
950 2010 l
1373 2030 m
1373 2010 l
1796 2030 m
1796 2010 l
2219 2030 m
2219 2010 l
2642 2030 m
2642 2010 l
/Times-Italic findfont 
60 scalefont
 setfont
/Helvetica findfont 
60 scalefont
 setfont
stroke
528 370 m
gsave
528 370 translate
0 rotate
0 -20  m
(0.0) CS
(0.0) show
grestore
newpath
950 370 m
gsave
950 370 translate
0 rotate
0 -20  m
(2.0) CS
(2.0) show
grestore
newpath
1373 370 m
gsave
1373 370 translate
0 rotate
0 -20  m
(4.0) CS
(4.0) show
grestore
newpath
1796 370 m
gsave
1796 370 translate
0 rotate
0 -20  m
(6.0) CS
(6.0) show
grestore
newpath
2219 370 m
gsave
2219 370 translate
0 rotate
0 -20  m
(8.0) CS
(8.0) show
grestore
newpath
2642 370 m
gsave
2642 370 translate
0 rotate
0 -20  m
(10.0) CS
(10.0) show
grestore
newpath
/Helvetica findfont 
60 scalefont
 setfont
1585 270 m
gsave
1585 270 translate
0 rotate
0 0  m
(H \(Tesla\)) CS
(H \(Tesla\)) show
grestore
newpath
528 420 m
538 420 l
528 581 m
538 581 l
528 742 m
538 742 l
528 903 m
538 903 l
528 1064 m
538 1064 l
528 1225 m
538 1225 l
528 1386 m
538 1386 l
528 1546 m
538 1546 l
528 1708 m
538 1708 l
528 1868 m
538 1868 l
528 2030 m
538 2030 l
2642 420 m
2632 420 l
2642 581 m
2632 581 l
2642 742 m
2632 742 l
2642 903 m
2632 903 l
2642 1064 m
2632 1064 l
2642 1225 m
2632 1225 l
2642 1386 m
2632 1386 l
2642 1546 m
2632 1546 l
2642 1708 m
2632 1708 l
2642 1868 m
2632 1868 l
2642 2030 m
2632 2030 l
stroke
528 420 m
548 420 l
528 742 m
548 742 l
528 1064 m
548 1064 l
528 1386 m
548 1386 l
528 1708 m
548 1708 l
528 2030 m
548 2030 l
2642 420 m
2622 420 l
2642 742 m
2622 742 l
2642 1064 m
2622 1064 l
2642 1386 m
2622 1386 l
2642 1708 m
2622 1708 l
2642 2030 m
2622 2030 l
/Helvetica findfont 
60 scalefont
 setfont
stroke
490 420 m
gsave
490 420 translate
0 rotate
0 -20  m
(0.0) RJ
(0.0) show
grestore
newpath
490 742 m
gsave
490 742 translate
0 rotate
0 -20  m
(10.0) RJ
(10.0) show
grestore
newpath
490 1064 m
gsave
490 1064 translate
0 rotate
0 -20  m
(20.0) RJ
(20.0) show
grestore
newpath
490 1386 m
gsave
490 1386 translate
0 rotate
0 -20  m
(30.0) RJ
(30.0) show
grestore
newpath
490 1708 m
gsave
490 1708 translate
0 rotate
0 -20  m
(40.0) RJ
(40.0) show
grestore
newpath
490 2030 m
gsave
490 2030 translate
0 rotate
0 -20  m
(50.0) RJ
(50.0) show
grestore
newpath
/Helvetica findfont 
60 scalefont
 setfont
317 1225 m
gsave
317 1225 translate
90 rotate
0 0  m
(F\(h,T\) \(s-1\)) CS
(F\(h,T\) \(s) show
/Helvetica findfont 
36 scalefont
 setfont
0 36 rmoveto
(-1) show
/Helvetica findfont 
60 scalefont
 setfont
0 -36 rmoveto
(\)) show
grestore
newpath
/Helvetica findfont 
90 scalefont
 setfont
1585 2198 m
gsave
1585 2198 translate
0 rotate
0 0  m
(Fermion F\(h,T\):) CS
(Fermion F\(h,T\):) show
grestore
newpath
/Helvetica findfont 
60 scalefont
 setfont
1585 2080 m
gsave
1585 2080 translate
0 rotate
0 0  m
(Contributions From The Uniform Part of the Spin   ) CS
(Contributions From The Uniform Part of the Spin   ) show
grestore
newpath
549 451 m
570 452 l
591 455 l
612 458 l
633 462 l
654 467 l
675 472 l
697 478 l
718 485 l
739 493 l
760 501 l
781 510 l
802 519 l
823 529 l
845 539 l
866 550 l
887 562 l
908 573 l
929 586 l
950 599 l
971 612 l
993 626 l
1014 640 l
1035 655 l
1056 671 l
1077 687 l
1098 705 l
1119 723 l
1141 743 l
1162 765 l
1183 789 l
1204 816 l
1225 847 l
1246 885 l
1267 936 l
1289 1017 l
1310 1286 l
1331 1021 l
1352 961 l
1373 927 l
1394 905 l
1415 890 l
1437 879 l
1458 871 l
1479 865 l
1500 860 l
1521 857 l
1542 855 l
1563 854 l
1585 853 l
1606 853 l
1627 854 l
1648 855 l
1669 856 l
1690 857 l
1711 859 l
1732 860 l
1754 862 l
1775 864 l
1796 866 l
1817 868 l
1838 870 l
1859 872 l
1880 875 l
1902 877 l
1923 879 l
1944 881 l
1965 882 l
1986 884 l
2007 886 l
2028 888 l
2050 889 l
2071 891 l
2092 892 l
2113 894 l
2134 895 l
2155 896 l
2176 897 l
2198 898 l
2219 899 l
2240 899 l
2261 900 l
2282 900 l
2303 901 l
2324 901 l
2346 901 l
2367 901 l
2388 900 l
2409 900 l
2430 899 l
stroke
[4 8] 0 setdash
549 474 m
570 476 l
591 478 l
612 482 l
633 486 l
654 491 l
675 497 l
697 504 l
718 511 l
739 519 l
760 528 l
781 538 l
802 548 l
823 558 l
845 569 l
866 581 l
887 594 l
908 606 l
929 620 l
950 634 l
971 648 l
993 663 l
1014 678 l
1035 695 l
1056 711 l
1077 729 l
1098 748 l
1119 767 l
1141 788 l
1162 811 l
1183 836 l
1204 864 l
1225 896 l
1246 934 l
1267 985 l
1289 1066 l
1310 1333 l
1331 1070 l
1352 1012 l
1373 979 l
1394 958 l
1415 942 l
1437 931 l
1458 923 l
1479 916 l
1500 911 l
1521 908 l
1542 905 l
1563 903 l
1585 902 l
1606 901 l
1627 900 l
1648 900 l
1669 900 l
1690 901 l
1711 902 l
1732 902 l
1754 903 l
1775 904 l
1796 905 l
1817 907 l
1838 908 l
1859 909 l
1880 910 l
1902 911 l
1923 913 l
1944 914 l
1965 915 l
1986 916 l
2007 917 l
2028 917 l
2050 918 l
2071 919 l
2092 919 l
2113 920 l
2134 920 l
2155 920 l
2176 920 l
2198 920 l
2219 920 l
2240 920 l
2261 919 l
2282 919 l
2303 918 l
2324 917 l
2346 916 l
2367 914 l
2388 913 l
2409 911 l
2430 909 l
stroke
[] 0 setdash
[20 20] 0 setdash
549 539 m
570 540 l
591 543 l
612 547 l
633 551 l
654 557 l
675 563 l
697 571 l
718 579 l
739 587 l
760 597 l
781 607 l
802 618 l
823 629 l
845 641 l
866 654 l
887 667 l
908 681 l
929 695 l
950 710 l
971 725 l
993 741 l
1014 757 l
1035 774 l
1056 792 l
1077 810 l
1098 829 l
1119 849 l
1141 871 l
1162 894 l
1183 919 l
1204 946 l
1225 978 l
1246 1016 l
1267 1065 l
1289 1144 l
1310 1408 l
1331 1148 l
1352 1092 l
1373 1060 l
1394 1039 l
1415 1024 l
1437 1012 l
1458 1003 l
1479 996 l
1500 990 l
1521 985 l
1542 980 l
1563 977 l
1585 974 l
1606 971 l
1627 968 l
1648 966 l
1669 964 l
1690 962 l
1711 960 l
1732 959 l
1754 957 l
1775 955 l
1796 954 l
1817 952 l
1838 950 l
1859 948 l
1880 946 l
1902 945 l
1923 943 l
1944 940 l
1965 938 l
1986 936 l
2007 934 l
2028 931 l
2050 929 l
2071 926 l
2092 923 l
2113 920 l
2134 917 l
2155 914 l
2176 910 l
2198 907 l
2219 903 l
2240 900 l
2261 896 l
2282 892 l
2303 887 l
2324 883 l
2346 879 l
2367 874 l
2388 869 l
2409 864 l
2430 859 l
stroke
[] 0 setdash
7 setlinewidth
549 504 m
570 562 l
591 637 l
612 715 l
633 785 l
654 844 l
675 892 l
697 929 l
718 957 l
739 979 l
760 995 l
781 1008 l
802 1017 l
823 1025 l
845 1030 l
866 1035 l
887 1038 l
908 1040 l
929 1042 l
950 1043 l
971 1044 l
993 1044 l
1014 1044 l
1035 1044 l
1056 1044 l
1077 1044 l
1098 1043 l
1119 1042 l
1141 1041 l
1162 1040 l
1183 1039 l
1204 1038 l
1225 1037 l
1246 1036 l
1267 1034 l
1289 1033 l
1310 1031 l
1331 1030 l
1352 1028 l
1373 1027 l
1394 1025 l
1415 1023 l
1437 1022 l
1458 1020 l
1479 1018 l
1500 1016 l
1521 1014 l
1542 1012 l
1563 1010 l
1585 1008 l
1606 1006 l
1627 1003 l
1648 1001 l
1669 998 l
1690 995 l
1711 993 l
1732 990 l
1754 986 l
1775 983 l
1796 980 l
1817 976 l
1838 972 l
1859 967 l
1880 963 l
1902 958 l
1923 953 l
1944 947 l
1965 941 l
1986 934 l
2007 927 l
2028 920 l
2050 912 l
2071 903 l
2092 894 l
2113 884 l
2134 873 l
2155 862 l
2176 850 l
2198 837 l
2219 824 l
2240 809 l
2261 794 l
2282 779 l
2303 762 l
2324 745 l
2346 728 l
2367 710 l
2388 691 l
2409 672 l
2430 653 l
stroke
1 setlinewidth
7 setlinewidth
[4 8] 0 setdash
549 553 m
570 617 l
591 699 l
612 784 l
633 860 l
654 923 l
675 973 l
697 1011 l
718 1038 l
739 1058 l
760 1072 l
781 1081 l
802 1087 l
823 1091 l
845 1093 l
866 1093 l
887 1093 l
908 1092 l
929 1091 l
950 1090 l
971 1088 l
993 1086 l
1014 1084 l
1035 1082 l
1056 1080 l
1077 1078 l
1098 1075 l
1119 1073 l
1141 1071 l
1162 1069 l
1183 1066 l
1204 1064 l
1225 1062 l
1246 1059 l
1267 1057 l
1289 1054 l
1310 1052 l
1331 1049 l
1352 1046 l
1373 1044 l
1394 1041 l
1415 1038 l
1437 1035 l
1458 1032 l
1479 1029 l
1500 1025 l
1521 1022 l
1542 1018 l
1563 1015 l
1585 1011 l
1606 1007 l
1627 1002 l
1648 998 l
1669 994 l
1690 989 l
1711 984 l
1732 978 l
1754 973 l
1775 967 l
1796 961 l
1817 955 l
1838 948 l
1859 942 l
1880 934 l
1902 927 l
1923 919 l
1944 911 l
1965 902 l
1986 893 l
2007 884 l
2028 874 l
2050 864 l
2071 854 l
2092 843 l
2113 832 l
2134 820 l
2155 809 l
2176 796 l
2198 784 l
2219 771 l
2240 758 l
2261 745 l
2282 731 l
2303 717 l
2324 703 l
2346 689 l
2367 675 l
2388 661 l
2409 647 l
2430 632 l
stroke
[] 0 setdash
1 setlinewidth
7 setlinewidth
[20 20] 0 setdash
549 675 m
570 745 l
591 837 l
612 932 l
633 1018 l
654 1090 l
675 1146 l
697 1187 l
718 1217 l
739 1236 l
760 1248 l
781 1253 l
802 1254 l
823 1252 l
845 1247 l
866 1240 l
887 1231 l
908 1222 l
929 1212 l
950 1202 l
971 1191 l
993 1180 l
1014 1170 l
1035 1159 l
1056 1148 l
1077 1138 l
1098 1128 l
1119 1117 l
1141 1107 l
1162 1098 l
1183 1088 l
1204 1079 l
1225 1069 l
1246 1060 l
1267 1051 l
1289 1042 l
1310 1034 l
1331 1025 l
1352 1016 l
1373 1008 l
1394 1000 l
1415 992 l
1437 983 l
1458 975 l
1479 967 l
1500 959 l
1521 951 l
1542 943 l
1563 936 l
1585 928 l
1606 920 l
1627 912 l
1648 904 l
1669 896 l
1690 888 l
1711 881 l
1732 873 l
1754 865 l
1775 857 l
1796 849 l
1817 841 l
1838 833 l
1859 825 l
1880 817 l
1902 809 l
1923 801 l
1944 794 l
1965 786 l
1986 778 l
2007 770 l
2028 762 l
2050 754 l
2071 746 l
2092 738 l
2113 730 l
2134 722 l
2155 714 l
2176 706 l
2198 698 l
2219 691 l
2240 683 l
2261 675 l
2282 667 l
2303 659 l
2324 652 l
2346 644 l
2367 636 l
2388 628 l
2409 621 l
2430 612 l
stroke
[] 0 setdash
1 setlinewidth
/Helvetica findfont 
60 scalefont
 setfont
/Helvetica findfont 
60 scalefont
 setfont
2489 1914 m
2629 1914 l
stroke
2664 1914 m
gsave
2664 1914 translate
0 rotate
0 -20  m
(H) show
/Helvetica findfont 
36 scalefont
 setfont
0 -18 rmoveto
(||a) show
/Helvetica findfont 
60 scalefont
 setfont
0 18 rmoveto
( at 1.4 K) show
grestore
newpath
/Helvetica findfont 
60 scalefont
 setfont
[4 8] 0 setdash
2489 1840 m
2629 1840 l
stroke
[] 0 setdash
2664 1840 m
gsave
2664 1840 translate
0 rotate
0 -20  m
(H) show
/Helvetica findfont 
36 scalefont
 setfont
0 -18 rmoveto
(||a) show
/Helvetica findfont 
60 scalefont
 setfont
0 18 rmoveto
( at 2.0 K) show
grestore
newpath
/Helvetica findfont 
60 scalefont
 setfont
[20 20] 0 setdash
2489 1766 m
2629 1766 l
stroke
[] 0 setdash
2664 1766 m
gsave
2664 1766 translate
0 rotate
0 -20  m
(H) show
/Helvetica findfont 
36 scalefont
 setfont
0 -18 rmoveto
(||a) show
/Helvetica findfont 
60 scalefont
 setfont
0 18 rmoveto
( at 4.2 K) show
grestore
newpath
/Helvetica findfont 
60 scalefont
 setfont
7 setlinewidth
2489 1692 m
2629 1692 l
stroke
1 setlinewidth
2664 1692 m
gsave
2664 1692 translate
0 rotate
0 -20  m
(H) show
/Helvetica findfont 
36 scalefont
 setfont
0 -18 rmoveto
(||b) show
/Helvetica findfont 
60 scalefont
 setfont
0 18 rmoveto
( at 1.4 K) show
grestore
newpath
/Helvetica findfont 
60 scalefont
 setfont
[4 8] 0 setdash
7 setlinewidth
2489 1618 m
2629 1618 l
stroke
[] 0 setdash
1 setlinewidth
2664 1618 m
gsave
2664 1618 translate
0 rotate
0 -20  m
(H) show
/Helvetica findfont 
36 scalefont
 setfont
0 -18 rmoveto
(||b) show
/Helvetica findfont 
60 scalefont
 setfont
0 18 rmoveto
( at 2.0 K) show
grestore
newpath
/Helvetica findfont 
60 scalefont
 setfont
[20 20] 0 setdash
7 setlinewidth
2489 1544 m
2629 1544 l
stroke
[] 0 setdash
1 setlinewidth
2664 1544 m
gsave
2664 1544 translate
0 rotate
0 -20  m
(H) show
/Helvetica findfont 
36 scalefont
 setfont
0 -18 rmoveto
(||b) show
/Helvetica findfont 
60 scalefont
 setfont
0 18 rmoveto
( at 4.2 K) show
grestore
newpath
showpage
%%Trailer


==> fig6 <==
%Figure6
%!PostScript
%%BoundingBox: 18 18 552 711
%%Creator: Xvgr version 2.10 - PJ Turner OGI-ESE
%%EndComments
/m {moveto} bind def
/l {lineto} bind def
/RJ {
 stringwidth neg exch neg exch
 rmoveto
} bind def
/CS {
 stringwidth
 2 div neg exch 2 div neg exch
 rmoveto
} bind def
0.25 0.25 scale
1 setlinecap
2450 0 translate
90 rotate
/Times-Italic findfont 
60 scalefont
 setfont
[] 0 setdash
519 420 m
519 2030 l
2595 2030 l
2595 420 l
519 420 l
stroke
[] 0 setdash
519 420 m
519 430 l
727 420 m
727 430 l
934 420 m
934 430 l
1142 420 m
1142 430 l
1349 420 m
1349 430 l
1557 420 m
1557 430 l
1765 420 m
1765 430 l
1972 420 m
1972 430 l
2180 420 m
2180 430 l
2387 420 m
2387 430 l
2595 420 m
2595 430 l
519 2030 m
519 2020 l
727 2030 m
727 2020 l
934 2030 m
934 2020 l
1142 2030 m
1142 2020 l
1349 2030 m
1349 2020 l
1557 2030 m
1557 2020 l
1765 2030 m
1765 2020 l
1972 2030 m
1972 2020 l
2180 2030 m
2180 2020 l
2387 2030 m
2387 2020 l
2595 2030 m
2595 2020 l
stroke
519 420 m
519 440 l
934 420 m
934 440 l
1349 420 m
1349 440 l
1765 420 m
1765 440 l
2180 420 m
2180 440 l
2595 420 m
2595 440 l
519 2030 m
519 2010 l
934 2030 m
934 2010 l
1349 2030 m
1349 2010 l
1765 2030 m
1765 2010 l
2180 2030 m
2180 2010 l
2595 2030 m
2595 2010 l
/Times-Italic findfont 
60 scalefont
 setfont
/Helvetica findfont 
60 scalefont
 setfont
stroke
519 370 m
gsave
519 370 translate
0 rotate
0 -20  m
(0.0) CS
(0.0) show
grestore
newpath
934 370 m
gsave
934 370 translate
0 rotate
0 -20  m
(2.0) CS
(2.0) show
grestore
newpath
1349 370 m
gsave
1349 370 translate
0 rotate
0 -20  m
(4.0) CS
(4.0) show
grestore
newpath
1765 370 m
gsave
1765 370 translate
0 rotate
0 -20  m
(6.0) CS
(6.0) show
grestore
newpath
2180 370 m
gsave
2180 370 translate
0 rotate
0 -20  m
(8.0) CS
(8.0) show
grestore
newpath
2595 370 m
gsave
2595 370 translate
0 rotate
0 -20  m
(10.0) CS
(10.0) show
grestore
newpath
/Helvetica findfont 
60 scalefont
 setfont
1557 270 m
gsave
1557 270 translate
0 rotate
0 0  m
(H \(Tesla\)) CS
(H \(Tesla\)) show
grestore
newpath
519 420 m
529 420 l
519 581 m
529 581 l
519 742 m
529 742 l
519 903 m
529 903 l
519 1064 m
529 1064 l
519 1225 m
529 1225 l
519 1386 m
529 1386 l
519 1546 m
529 1546 l
519 1708 m
529 1708 l
519 1868 m
529 1868 l
519 2030 m
529 2030 l
2595 420 m
2585 420 l
2595 581 m
2585 581 l
2595 742 m
2585 742 l
2595 903 m
2585 903 l
2595 1064 m
2585 1064 l
2595 1225 m
2585 1225 l
2595 1386 m
2585 1386 l
2595 1546 m
2585 1546 l
2595 1708 m
2585 1708 l
2595 1868 m
2585 1868 l
2595 2030 m
2585 2030 l
stroke
519 420 m
539 420 l
519 742 m
539 742 l
519 1064 m
539 1064 l
519 1386 m
539 1386 l
519 1708 m
539 1708 l
519 2030 m
539 2030 l
2595 420 m
2575 420 l
2595 742 m
2575 742 l
2595 1064 m
2575 1064 l
2595 1386 m
2575 1386 l
2595 1708 m
2575 1708 l
2595 2030 m
2575 2030 l
/Helvetica findfont 
60 scalefont
 setfont
stroke
481 420 m
gsave
481 420 translate
0 rotate
0 -20  m
(0.0) RJ
(0.0) show
grestore
newpath
481 742 m
gsave
481 742 translate
0 rotate
0 -20  m
(10.0) RJ
(10.0) show
grestore
newpath
481 1064 m
gsave
481 1064 translate
0 rotate
0 -20  m
(20.0) RJ
(20.0) show
grestore
newpath
481 1386 m
gsave
481 1386 translate
0 rotate
0 -20  m
(30.0) RJ
(30.0) show
grestore
newpath
481 1708 m
gsave
481 1708 translate
0 rotate
0 -20  m
(40.0) RJ
(40.0) show
grestore
newpath
481 2030 m
gsave
481 2030 translate
0 rotate
0 -20  m
(50.0) RJ
(50.0) show
grestore
newpath
/Helvetica findfont 
60 scalefont
 setfont
308 1225 m
gsave
308 1225 translate
90 rotate
0 0  m
(F\(h,T\) \(s-1\)) CS
(F\(h,T\) \(s) show
/Helvetica findfont 
36 scalefont
 setfont
0 36 rmoveto
(-1) show
/Helvetica findfont 
60 scalefont
 setfont
0 -36 rmoveto
(\)) show
grestore
newpath
/Helvetica findfont 
90 scalefont
 setfont
1557 2198 m
gsave
1557 2198 translate
0 rotate
0 0  m
(Fermion F\(h,T\):) CS
(Fermion F\(h,T\):) show
grestore
newpath
/Helvetica findfont 
60 scalefont
 setfont
1557 2080 m
gsave
1557 2080 translate
0 rotate
0 0  m
(Contributions From The Uniform Part of the Spin   ) CS
(Contributions From The Uniform Part of the Spin   ) show
grestore
newpath
540 450 m
561 451 l
582 452 l
602 454 l
623 456 l
644 459 l
665 461 l
685 465 l
706 468 l
727 472 l
748 476 l
768 480 l
789 485 l
810 490 l
831 495 l
851 500 l
872 506 l
893 511 l
914 517 l
934 523 l
955 529 l
976 536 l
997 542 l
1017 548 l
1038 555 l
1059 561 l
1080 568 l
1100 575 l
1121 581 l
1142 588 l
1163 594 l
1183 601 l
1204 607 l
1225 614 l
1246 620 l
1266 627 l
1287 633 l
1308 639 l
1329 645 l
1349 651 l
1370 657 l
1391 663 l
1412 669 l
1432 675 l
1453 680 l
1474 685 l
1495 691 l
1515 696 l
1536 701 l
1557 706 l
1578 710 l
1599 715 l
1619 720 l
1640 724 l
1661 728 l
1682 732 l
1702 736 l
1723 740 l
1744 743 l
1765 747 l
1785 750 l
1806 753 l
1827 756 l
1848 759 l
1868 762 l
1889 765 l
1910 767 l
1931 769 l
1951 771 l
1972 773 l
1993 775 l
2014 777 l
2034 779 l
2055 780 l
2076 781 l
2097 782 l
2117 783 l
2138 784 l
2159 784 l
2180 785 l
2200 785 l
2221 785 l
2242 785 l
2263 784 l
2283 784 l
2304 783 l
2325 782 l
2346 781 l
2366 779 l
2387 778 l
stroke
[4 8] 0 setdash
540 474 m
561 474 l
582 476 l
602 477 l
623 479 l
644 482 l
665 485 l
685 488 l
706 491 l
727 495 l
748 499 l
768 503 l
789 508 l
810 513 l
831 518 l
851 523 l
872 528 l
893 534 l
914 540 l
934 546 l
955 552 l
976 558 l
997 564 l
1017 570 l
1038 577 l
1059 583 l
1080 590 l
1100 596 l
1121 603 l
1142 609 l
1163 615 l
1183 622 l
1204 628 l
1225 635 l
1246 641 l
1266 647 l
1287 653 l
1308 659 l
1329 665 l
1349 671 l
1370 677 l
1391 683 l
1412 688 l
1432 694 l
1453 699 l
1474 705 l
1495 710 l
1515 715 l
1536 719 l
1557 724 l
1578 729 l
1599 733 l
1619 737 l
1640 741 l
1661 745 l
1682 749 l
1702 753 l
1723 756 l
1744 760 l
1765 763 l
1785 766 l
1806 769 l
1827 771 l
1848 774 l
1868 776 l
1889 778 l
1910 780 l
1931 782 l
1951 784 l
1972 785 l
1993 787 l
2014 788 l
2034 789 l
2055 789 l
2076 790 l
2097 790 l
2117 790 l
2138 790 l
2159 790 l
2180 789 l
2200 789 l
2221 788 l
2242 786 l
2263 785 l
2283 783 l
2304 781 l
2325 779 l
2346 777 l
2366 774 l
2387 771 l
stroke
[] 0 setdash
[20 20] 0 setdash
540 538 m
561 539 l
582 540 l
602 542 l
623 544 l
644 546 l
665 549 l
685 552 l
706 555 l
727 558 l
748 562 l
768 566 l
789 570 l
810 575 l
831 580 l
851 584 l
872 589 l
893 594 l
914 600 l
934 605 l
955 610 l
976 616 l
997 621 l
1017 627 l
1038 633 l
1059 638 l
1080 644 l
1100 649 l
1121 655 l
1142 660 l
1163 666 l
1183 671 l
1204 676 l
1225 682 l
1246 687 l
1266 692 l
1287 697 l
1308 701 l
1329 706 l
1349 710 l
1370 715 l
1391 719 l
1412 723 l
1432 727 l
1453 730 l
1474 734 l
1495 737 l
1515 740 l
1536 743 l
1557 746 l
1578 749 l
1599 751 l
1619 753 l
1640 756 l
1661 757 l
1682 759 l
1702 761 l
1723 762 l
1744 763 l
1765 764 l
1785 765 l
1806 766 l
1827 766 l
1848 766 l
1868 766 l
1889 766 l
1910 766 l
1931 765 l
1951 764 l
1972 763 l
1993 762 l
2014 761 l
2034 760 l
2055 758 l
2076 756 l
2097 754 l
2117 752 l
2138 750 l
2159 747 l
2180 745 l
2200 742 l
2221 739 l
2242 735 l
2263 732 l
2283 729 l
2304 725 l
2325 721 l
2346 717 l
2366 713 l
2387 709 l
stroke
[] 0 setdash
7 setlinewidth
540 504 m
561 562 l
582 637 l
602 715 l
623 785 l
644 844 l
665 892 l
685 929 l
706 957 l
727 979 l
748 995 l
768 1008 l
789 1017 l
810 1025 l
831 1030 l
851 1035 l
872 1038 l
893 1040 l
914 1042 l
934 1043 l
955 1044 l
976 1044 l
997 1044 l
1017 1044 l
1038 1044 l
1059 1044 l
1080 1043 l
1100 1042 l
1121 1041 l
1142 1040 l
1163 1039 l
1183 1038 l
1204 1037 l
1225 1036 l
1246 1034 l
1266 1033 l
1287 1031 l
1308 1030 l
1329 1028 l
1349 1027 l
1370 1025 l
1391 1023 l
1412 1022 l
1432 1020 l
1453 1018 l
1474 1016 l
1495 1014 l
1515 1012 l
1536 1010 l
1557 1008 l
1578 1006 l
1599 1003 l
1619 1001 l
1640 998 l
1661 995 l
1682 993 l
1702 990 l
1723 986 l
1744 983 l
1765 980 l
1785 976 l
1806 972 l
1827 967 l
1848 963 l
1868 958 l
1889 953 l
1910 947 l
1931 941 l
1951 934 l
1972 927 l
1993 920 l
2014 912 l
2034 903 l
2055 894 l
2076 884 l
2097 873 l
2117 862 l
2138 850 l
2159 837 l
2180 824 l
2200 809 l
2221 794 l
2242 779 l
2263 762 l
2283 745 l
2304 728 l
2325 710 l
2346 691 l
2366 672 l
2387 653 l
stroke
1 setlinewidth
7 setlinewidth
[4 8] 0 setdash
540 553 m
561 617 l
582 699 l
602 784 l
623 860 l
644 923 l
665 973 l
685 1011 l
706 1038 l
727 1058 l
748 1072 l
768 1081 l
789 1087 l
810 1091 l
831 1093 l
851 1093 l
872 1093 l
893 1092 l
914 1091 l
934 1090 l
955 1088 l
976 1086 l
997 1084 l
1017 1082 l
1038 1080 l
1059 1078 l
1080 1075 l
1100 1073 l
1121 1071 l
1142 1069 l
1163 1066 l
1183 1064 l
1204 1062 l
1225 1059 l
1246 1057 l
1266 1054 l
1287 1052 l
1308 1049 l
1329 1046 l
1349 1044 l
1370 1041 l
1391 1038 l
1412 1035 l
1432 1032 l
1453 1029 l
1474 1025 l
1495 1022 l
1515 1018 l
1536 1015 l
1557 1011 l
1578 1007 l
1599 1002 l
1619 998 l
1640 994 l
1661 989 l
1682 984 l
1702 978 l
1723 973 l
1744 967 l
1765 961 l
1785 955 l
1806 948 l
1827 942 l
1848 934 l
1868 927 l
1889 919 l
1910 911 l
1931 902 l
1951 893 l
1972 884 l
1993 874 l
2014 864 l
2034 854 l
2055 843 l
2076 832 l
2097 820 l
2117 809 l
2138 796 l
2159 784 l
2180 771 l
2200 758 l
2221 745 l
2242 731 l
2263 717 l
2283 703 l
2304 689 l
2325 675 l
2346 661 l
2366 647 l
2387 632 l
stroke
[] 0 setdash
1 setlinewidth
7 setlinewidth
[20 20] 0 setdash
540 675 m
561 745 l
582 837 l
602 932 l
623 1018 l
644 1090 l
665 1146 l
685 1187 l
706 1217 l
727 1236 l
748 1248 l
768 1253 l
789 1254 l
810 1252 l
831 1247 l
851 1240 l
872 1231 l
893 1222 l
914 1212 l
934 1202 l
955 1191 l
976 1180 l
997 1170 l
1017 1159 l
1038 1148 l
1059 1138 l
1080 1128 l
1100 1117 l
1121 1107 l
1142 1098 l
1163 1088 l
1183 1079 l
1204 1069 l
1225 1060 l
1246 1051 l
1266 1042 l
1287 1034 l
1308 1025 l
1329 1016 l
1349 1008 l
1370 1000 l
1391 992 l
1412 983 l
1432 975 l
1453 967 l
1474 959 l
1495 951 l
1515 943 l
1536 936 l
1557 928 l
1578 920 l
1599 912 l
1619 904 l
1640 896 l
1661 888 l
1682 881 l
1702 873 l
1723 865 l
1744 857 l
1765 849 l
1785 841 l
1806 833 l
1827 825 l
1848 817 l
1868 809 l
1889 801 l
1910 794 l
1931 786 l
1951 778 l
1972 770 l
1993 762 l
2014 754 l
2034 746 l
2055 738 l
2076 730 l
2097 722 l
2117 714 l
2138 706 l
2159 698 l
2180 691 l
2200 683 l
2221 675 l
2242 667 l
2263 659 l
2283 652 l
2304 644 l
2325 636 l
2346 628 l
2366 621 l
2387 612 l
stroke
[] 0 setdash
1 setlinewidth
/Helvetica findfont 
60 scalefont
 setfont
/Helvetica findfont 
60 scalefont
 setfont
2400 1914 m
2540 1914 l
stroke
2575 1914 m
gsave
2575 1914 translate
0 rotate
0 -20  m
(H) show
/Helvetica findfont 
36 scalefont
 setfont
0 -18 rmoveto
(||c) show
/Helvetica findfont 
60 scalefont
 setfont
0 18 rmoveto
( at 1.4 K) show
grestore
newpath
/Helvetica findfont 
60 scalefont
 setfont
[4 8] 0 setdash
2400 1840 m
2540 1840 l
stroke
[] 0 setdash
2575 1840 m
gsave
2575 1840 translate
0 rotate
0 -20  m
(H) show
/Helvetica findfont 
36 scalefont
 setfont
0 -18 rmoveto
(||c) show
/Helvetica findfont 
60 scalefont
 setfont
0 18 rmoveto
( at 2.0 K) show
grestore
newpath
/Helvetica findfont 
60 scalefont
 setfont
[20 20] 0 setdash
2400 1766 m
2540 1766 l
stroke
[] 0 setdash
2575 1766 m
gsave
2575 1766 translate
0 rotate
0 -20  m
(H) show
/Helvetica findfont 
36 scalefont
 setfont
0 -18 rmoveto
(||c) show
/Helvetica findfont 
60 scalefont
 setfont
0 18 rmoveto
( at 4.2 K) show
grestore
newpath
/Helvetica findfont 
60 scalefont
 setfont
7 setlinewidth
2400 1692 m
2540 1692 l
stroke
1 setlinewidth
2575 1692 m
gsave
2575 1692 translate
0 rotate
0 -20  m
(H) show
/Helvetica findfont 
36 scalefont
 setfont
0 -18 rmoveto
(||b) show
/Helvetica findfont 
60 scalefont
 setfont
0 18 rmoveto
( at 1.4 K) show
grestore
newpath
/Helvetica findfont 
60 scalefont
 setfont
[4 8] 0 setdash
7 setlinewidth
2400 1618 m
2540 1618 l
stroke
[] 0 setdash
1 setlinewidth
2575 1618 m
gsave
2575 1618 translate
0 rotate
0 -20  m
(H) show
/Helvetica findfont 
36 scalefont
 setfont
0 -18 rmoveto
(||b) show
/Helvetica findfont 
60 scalefont
 setfont
0 18 rmoveto
( at 2.0 K) show
grestore
newpath
/Helvetica findfont 
60 scalefont
 setfont
[20 20] 0 setdash
7 setlinewidth
2400 1544 m
2540 1544 l
stroke
[] 0 setdash
1 setlinewidth
2575 1544 m
gsave
2575 1544 translate
0 rotate
0 -20  m
(H) show
/Helvetica findfont 
36 scalefont
 setfont
0 -18 rmoveto
(||b) show
/Helvetica findfont 
60 scalefont
 setfont
0 18 rmoveto
( at 4.2 K) show
grestore
newpath
showpage
%%Trailer

